Aging and memory effects in social and economic dynamics

In this doctoral thesis, we investigate the complex interplay between temporal dynamics associated with aging and memory and their effects on social and economic systems. To do so, we combine theoretical modeling, to explore the aging implications in threshold (peer pressure) models, and empirical analysis, to address the impact of temporal and spatial patterns in real complex systems, taking housing market as a case study.

==> Front/International.tex <==
Prof. Jos\'e Javier Ramasco of the Consejo Superior de Investigaciones Cient\'ificas (CSIC) and Prof. Maxi San Miguel of the Universitat de les Illes Balears (UIB)

\vspace*{2 cm}

WE DECLARE:

\vspace*{1 cm}

That the thesis titles \textit{Aging and memory effects in social and economic dynamics}, presented by David Abella Bujalance to obtain a doctoral degree, has been completed under my supervision and meets the requirements to opt for an International Doctorate.

\vspace*{1 cm}

For all intents and purposes, we hereby sign this document.

\vspace*{1 cm}

Signature

\vspace*{3.5 cm}

\rule{5.5cm}{0.4pt} \hfill \noindent\rule{5.5cm}{0.4pt}

\vspace*{0.1 cm}

      \textbf{Prof. Jos\'e Javier Ramasco Sukia}              \hfill  \textbf{Prof. Maxi San Miguel Ruibal}


\vspace*{0.1 cm}

        Thesis Supervisor              \hfill Thesis Supervisor

\vspace*{3.5 cm}

\rule{5.5cm}{0.4pt} \hfill \noindent\rule{5.5cm}{0.4pt}

\vspace*{0.1 cm}

\textbf{David Abella Bujalance}              \hfill  \textbf{Dr. Cristóbal López Sánchez}


\vspace*{0.1 cm}

        PhD candidate              \hfill    Thesis Tutor

\vspace*{1 cm}

        Palma de Mallorca, July 2024

\vfill
